GIARPS High-resolution Observations of T Tauri stars (GHOsT). II. Connecting atomic and molecular winds in protoplanetary disks

In the framework of the GIARPS High-resolution Observations of T Tauri stars (GHOsT) project, we aim to characterize the atomic and molecular winds in a sample of classical T Tauri stars (CTTs) of the Taurus-Auriga region. We analyzed the flux calibrated [OI] 630 nm and $\rm H_2$ 2.12 $\rm \mu m$ lines in a sample of 36 CTTs observed at the Telescopio Nazionale Galileo with the HARPS and GIANO spectrographs. We decomposed the line profiles into different kinematic Gaussian components and focused on the most frequently detected component, the narrow low-velocity (v$\rm_p < 20$ $\rm km$ $\rm s^{-1}$) component (NLVC). We found that the $\rm H_2$ line is detected in 17 sources ($\sim 50 \%$ detection rate), and [OI] is detected in all sources but one. The NLV components of the $\rm H_2$ and [OI] emission are kinematically linked, with a strong correlation between the peak velocities and the full widths at half maximum of the two lines. Assuming Keplerian broadening, we found that the [OI] NVLC originates from a disk region between 0.05 and 20 au and that of $\rm H_2$ in a region from 2 and 20 au. We did not find any clear correlation between v$\rm_p$ of the $\rm H_2$ and [OI] NVLC and the outer disk inclination. This result is in line with previous studies. Our results suggest that molecular and neutral atomic emission in disk winds originate from regions that might overlap, and that the survival of molecular winds in disks strongly depends on the gas exposure to the radiation from the central star. Our results demonstrate the potential of wide-band high-resolution spectroscopy in linking tracers of different manifestations of the same phenomenon.

==> Tables/ORDERED_by_coordinates/H2_OI_lum.tex <==
\begin{table*}
\center
\caption{\label{tab:H2_OI_lum} \htwo\ and \oi\ extinction-corrected luminosity. }
\begin{tabular}{lccc}
\hline
Source           & Obs Date          & \htwo\      					    & \oi\	  					 \\
                 &                   & [$10^{-5} \rm L_{\odot}$] 	& [$10^{-5} \rm L_{\odot}$]  \\
\hline
\hline   
 CW Tau          & 20 Dec 2015       & < 2.08           & -          		  \\ 
                 & 08 Dec 2018       & < 1.66           & 5.07 $\pm$ 0.23     \\ 
 V409 Tau        & 26 Gen 2020       & < 0.57		    & 0.17 $\pm$ 0.02 	  \\ 
 DD Tau          & 19 Dec 2015       & < 2.23           & -			 		  \\ 
 BP Tau          & 25 Gen 2020       & 3.31 $\pm$ 0.38  & 0.86 $\pm$ 0.08  	  \\ 	 
 RY Tau          & 20 Dec 2015       & < 7.05           & -      	 		  \\ 
                 & 13 Nov 2017       & < 7.13           & 8.15 $\pm$ 0.39  	  \\ 
 FT Tau          & 25 Gen 2020       & < 0.88		    & 0.16 $\pm$ 0.01	  \\ 
 IP Tau          & 09 Dec 2018       & < 1.27           & 0.24 $\pm$ 0.01     \\ 
 DF Tau          & 20 Dec 2015       & < 2.06           & -          		  \\ 
                 & 08 Dec 2018       & < 1.57           & 0.43 $\pm$ 0.02     \\ 
 DG Tau          & 20 Dec 2015       & 14.80 $\pm$ 0.72 & -  	 	 		  \\ 
                 & 29 Oct 2017       & 11.91 $\pm$ 0.56 & 12.08 $\pm$ 0.55	  \\     
 DH Tau          & 02 Nov 2019       & < 1.36           & 0.62 $\pm$ 0.07     \\ 
 IQ Tau          & 02 Nov 2019       & 1.72 $\pm$ 0.23  & 1.28 $\pm$ 0.14	  \\ 
 UX Tau          & 26 Gen 2020       & 1.24 $\pm$ 0.38	& 2.48 $\pm$ 0.23	  \\ 
 DK Tau          & 08 Dec 2018       & < 1.49           & 2.21 $\pm$ 0.11	  \\ 
 GG Tau          & 09 Dec 2018       & 3.69 $\pm$ 0.54  & 0.65 $\pm$ 0.05	  \\ 
 UZ Tau          & 09 Dec 2018       & 3.21 $\pm$ 0.21  & 6.63 $\pm$ 0.33	  \\ 
 GH Tau          & 25 Gen 2020       & < 1.19		    & 0.65 $\pm$ 0.06	  \\ 
 GI Tau          & 26 Gen 2020       & 7.02 $\pm$ 0.68  & 0.47 $\pm$ 0.04	  \\ 
 DL Tau          & 20 Dec 2015       & 11.10 $\pm$ 0.60 & -      	 		  \\
                 & 29 Oct 2017       & 9.34 $\pm$ 0.52  & 0.84 $\pm$ 0.04	  \\ 
 HN Tau          & 19 Dec 2015       & 5.28 $\pm$ 0.25  & -     	 		  \\
                 & 29 Oct 2017       & 3.86 $\pm$ 0.24  & 4.90 $\pm$ 0.22	  \\
 CI Tau          & 09 Dec 2018       & < 1.54           & 0.39 $\pm$ 0.02     \\
 HL Tau          & 24 Nov 2016       & -                & -		     		  \\
 XZ Tau          & 14 Mar 2017       & -     		    & -			 		  \\
 GK Tau          & 02 Nov 2019       & < 1.46           & 1.64 $\pm$ 0.16	  \\
 DN Tau          & 01 Nov 2019       & < 1.18           & 0.79 $\pm$ 0.10 	  \\ 
 HQ Tau          & 01 Nov 2019       & < 2.35           & 4.91 $\pm$ 0.47 	  \\ 
 CoKu HP Tau G2  & 25 Gen 2020       & < 2.08		    & -			 		  \\ 
 DO Tau          & 19 Dec 2015       & 2.57 $\pm$ 0.14  & -		     		  \\ 
                 & 13 Nov 2017       & 3.24 $\pm$ 0.38  & 1.95 $\pm$ 0.10	  \\ 
                 & 26 Gen 2020       & 3.50 $\pm$ 0.43  & 1.48 $\pm$ 0.15     \\    
 DQ Tau          & 02 Nov 2019       & < 1.54           & 6.63 $\pm$ 0.60 	  \\ 
 DR Tau          & 25 Gen 2020       & 12.54 $\pm$ 1.99 & 1.14 $\pm$ 0.12	  \\
 DS Tau	         & 01 Nov 2019       & 0.62 $\pm$ 0.12  & 0.52 $\pm$ 0.17     \\ 
 UY Aur          & 08 Dec 2018       & 7.77 $\pm$ 0.46  & 1.82 $\pm$ 0.12     \\ 
 GM Aur          & 09 Dec 2018       & 1.79 $\pm$ 0.20  & 0.44 $\pm$ 0.11	  \\ 
 MWC480          & 01 Nov 2019       & < 2.29           & 2.31 $\pm$ 0.85	  \\ 
 V836 Tau        & 02 Nov 2019       & < 1.20           & 0.66 $\pm$ 0.09	  \\		
 RW Aur A        & 13 Nov 2017       & 8.35 $\pm$ 0.74 - 6.42 $\pm$ 0.74$^{(1)}$     & - \\
 CQ Tau          & 13 Nov 2017       & < 5.60           & 4.05 $\pm$ 0.19  	  \\  
\hline
\end{tabular}
\begin{quotation}
\textbf{Notes.} (1) Different values are obtained for the adoption of different extinctions values.
\end{quotation}
\end{table*} 



==> Tables/ORDERED_by_coordinates/JournalOfObservations.tex <==
\begin{table*}
\small
\center
\caption{\label{tab:Logbook} Journal of observations and photometry.}
\begin{tabular}{lcccccccccc}
\hline
\hline
          &              & $t_{exp}$ & $t_{exp}$ &       &       &       &       &       &       &      \\
Source    & Obs Date     & HARPS     & GIANO     & $B$   & $V$   & $R$   & $I$   & $J$   & $H$   & $K$  \\
\hline
          &              & [s]       & [s]       & [mag] & [mag] & [mag] & [mag] & [mag] & [mag] & [mag] \\
\hline
\hline   
 BP Tau   & 26 Gen 2020  & 3000		 & 2400		 & -	 & -	 & - 	 & -	 & 9.14  & -	& 7.81 \\
 CI Tau   & 09 Dec 2018  & 3000      & 2400      & 14.30 & 12.94 & 11.97 & 10.97 & 9.45  & 8.44 & 7.86 \\
 CoKu HP  & 25 Gen 2020  & 3000		 & 2400		 & -	 & -	 & -	 & -	 & 8.18  & -	& 7.35 \\
 CQ Tau   & 13 Nov 2017  & 2200      & 1800      & 10.89 & 9.84  & 9.41  & 8.98  & 8.01  & 7.20 & 6.36 \\
 CW Tau   & 20 Dec 2015  & -         & 2400      & -     & -     & -     & -     & 9.10  & 7.82 & 6.74 \\ 
          & 08 Dec 2018  & 3000      & 2400      & 15.35 & 13.76 & 12.53 & 11.51 & 9.05  & 7.80 & 6.95 \\    
 DD Tau   & 19 Dec 2015  & -         & 2400      & -     & -     & -     & -     & 10.10 & 8.78 & 7.86 \\ 
 DF Tau   & 20 Dec 2015  & -         & 1800      & -     & -     & -     & -     & 8.02  & 7.14 & 6.62 \\
          & 08 Dec 2018  & 2200      & 1800      & 13.40 & 12.17 & 11.10 & 9.85  & 8.08  & 7.15 & 6.97 \\
 DG Tau   & 19 Dec 2015  & -         & 1800      & -     & -     & -     & -     & 8.51  & 7.30 & 6.36 \\
          & 29 Oct 2017  & 2200      & 1800      & 13.65 & 12.58 & 11.50 & 10.46 & -     & 7.66 & 6.80 \\
 DH Tau   & 02 Nov 2019  & 3000      & 2400      & -     & -     & -     & -     & 9.48  & -    & 7.92 \\
 DK Tau   & 08 Dec 2018  & 2200      & 1800      & 13.96 & 12.58 & 11.59 & 10.59 & 8.89  & 7.90 & 7.04 \\
 DL Tau   & 20 Dec 2015  & -         & 2400      & -     & -     & -     & -     & 9.46  & 8.46 & 7.78 \\
          & 29 Oct 2017  & 3000      & 2400      & 14.32 & 13.06 & 12.05 & 11.01 & 9.55  & 8.61 & 7.93 \\
 DN Tau   & 01 Nov 2019  & 3000      & 2400      & -     & -     & -     & -     & 9.13  & -    & 7.90 \\
 DO Tau   & 19 Dec 2015  & -         & 2400      & -     & -     & -     & -     & 9.89  & 8.61 & 7.57 \\
          & 13 Nov 2017  & 3000      & 2400      & 14.34 & 13.18 & 12.27 & 11.23 & 9.28  & 8.17 & 7.34 \\ 
          & 26 Gen 2020  & 3000      & 2400      & -     & -     & -     & -     & 9.29  & -    & 7.15 \\       
 DQ Tau   & 02 Nov 2019  & 3000      & 2400      & -     & -     & -     & -     & 9.52  & -    & 8.01 \\
 DR Tau   & 25 Gen 2020  & 2300		 & 1800		 & -	 & -	 & -	 & -	 & 8.89	 & -	& 6.80 \\
 DS Tau	  & 01 Nov 2019  & 3000      & 2400      & -     & -     & -     & -     & 10.31 & -    & 8.86 \\
 FT Tau   & 25 Gen 2020  & 4600		 & 3600		 & -	 & -	 & -	 & -	 & 10.29 & -	& 8.81 \\        
 GG Tau   & 09 Dec 2018  & 2200      & 1800      & 13.55 & 12.18 & 11.16 & 10.22 & 8.62  & 7.91 & 7.31 \\  
 GH Tau   & 25 Gen 2020  & 3000		 & 2400		 & -	 & -	 & -	 & -	 & 9.08	 & -	& 7.72 \\
 GI Tau   & 26 Gen 2020  & 3000		 & 2400		 & -	 & -	 & -	 & -	 & 9.56  & -    & 7.75 \\ 
 GK Tau   & 02 Nov 2019  & 3000      & 2400      & -     & -     & -     & -     & 8.89  & -    & 7.23 \\
 GM Aur   & 09 Dec 2018  & 3000      & 2400      & 13.41 & 12.30 & 11.44 & 10.71 & 9.49  & 8.79 & 8.61 \\
 HL Tau   & 24 Nov 2016  & -         & 1800      & -     & -     & -     & -     & -     & -    & -    \\
 HN Tau   & 19 Dec 2015  & -         & 3600      & -     & -     & -     & -     & 10.70 & 9.49 & 8.45 \\
          & 29 Oct 2017  & 4500      & 3600      & 15.00 & 13.99 & 13.12 & 12.27 & 10.82 & 9.79 & 8.78 \\
 HQ Tau   & 01 Nov 2019  & 2300      & 1800      & -     & -     & -     & -     & 8.65  & -    & 7.13 \\
 IP Tau   & 09 Dec 2018  & 3000      & 2400      & 14.35 & 13.14 & 12.22 & 11.21 & 9.76  & 8.88 & 8.39 \\
 IQ Tau   & 02 Nov 2019  & 3000      & 3600      & -     & -     & -     & -     & -     & -    & 8.00 \\
 MWC480   & 01 Nov 2019  & 960       & 1200      & -     & -     & -     & -     & 7.82  & -    & 6.59 \\
 RW Aur A & 13 Nov 2017  & 2200      & 1800      & 11.04 & 10.44 & 9.97  & 9.38  & 8.41  & 7.66 & 7.06 \\
 RY Tau   & 20 Dec 2015  & -         & 1200      & -     & -     & -     & -     & 7.40  & 6.30 & 5.40 \\
          & 13 Nov 2017  & 1500      & 1200      & 11.49 & 10.36 & 9.61  & 8.81  & 6.95  & 6.45 & 5.84 \\
 UX Tau   & 26 Gen 2020  & 2280		 & 1800		 & -	 & -	 & -	 & -	 & 9.08  & - 	& 7.78 \\
 UY Aur   & 08 Dec 2018  & 2200      & 1800      & 13.99 & 12.72 & 11.71 & 10.78 & 9.15  & 8.07 & 7.15 \\
 UZ Tau   & 09 Dec 2018  & 3755      & 3000      & 14.31 & 12.87 & 11.70 & 10.34 & 9.33  & 8.41 & 7.98 \\
 V409 Tau & 26 Gen 2020  & 4600		 & 3600		 & -	 & -	 & -	 & -	 & 9.79  & -	& 8.44 \\
 V836 Tau & 02 Nov 2019  & 3000      & 2400      & -     & -     & -     & -     & 9.91  & -    & 8.59 \\
 XZ Tau   & 14 Mar 2017  & 1800      & 3000      & -     & -     & -     & -     & -     & -    & -    \\
\hline\end{tabular}
\begin{quotation}
\textbf{Notes.} Typical errors in photometric magnitudes are 0.01 mag in the optical bands, 0.05 in the NIR bands for data taken in 2015,2017,2018 and 0.1 mag in the NIR bands for data taken in 2019-2020.
\end{quotation}
\end{table*} 


==> Tables/ORDERED_by_coordinates/LineKinematicParameters.tex <==
\begin{table*}
\center
\caption{\label{tab:KinematicParameters} Line kinematic parameters of the NLVC for the \oi\ and \htwo\ profiles.}
\begin{tabular}{lc|ccc|ccc}
\hline
\hline
          &             & \multicolumn{3}{c}{NLVC - \oi}                     & \multicolumn{3}{c}{NLVC - \htwo}		                 \\	
Source    & Obs Date    & $\rm v_p$             & $\rm FWHM$           & $\rm I_p$           & $\rm v_p$             & $\rm FWHM$           & $\rm I_p$              \\
\hline   
 CW Tau   & 20 Dec 2015 & -                 & -                 & -                 & ND                & ND               & ND                 \\  
          & 08 Dec 2018 & 1.59 $\pm$ 4.21   & 35.22 $\pm$ 8.40  & 28.50 $\pm$ 3.00  & ND                & ND               & ND                 \\ 
 V409 Tau & 26 Gen 2020 & 21.00 $\pm$ 12.92 & 54.10 $\pm$ 42.90 & 1.20  $\pm$ 0.40  & ND                & ND               & ND                 \\  
 DD Tau   & 19 Dec 2015 & -                 & -                 & -                 & -19.07 $\pm$ 2.02 & 12.48 $\pm$ 0.73 & 42.00 $\pm$ 1.80   \\
 BP Tau   & 26 Gen 2020 & 2.50 $\pm$ 2.17   & 31.69 $\pm$ 4.36  & 16.40 $\pm$ 2.10  & 5.65 $\pm$ 2.37   & 27.32 $\pm$ 5.58 & 23.20 $\pm$ 3.10   \\  
 RY Tau   & 20 Dec 2015 & -                 & -                 & -                 & ND                & ND               & ND                 \\ 
          & 13 Nov 2017 & -10.40 $\pm$ 6.16 & 38.91 $\pm$ 11.82 & 42.40 $\pm$ 9.40  & ND                & ND               & ND                 \\ 
 FT Tau   & 25 Gen 2020 & -18.00 $\pm$ 8.00 & 37.59 $\pm$ 10.60 & 1.30  $\pm$ 0.30  & ND                & ND               & ND                 \\  
 IP Tau   & 09 Dec 2018 & -36.72 $\pm$ 2.36 & 43.92 $\pm$ 1.84  & 2.60  $\pm$ 0.68  & ND                & ND               & ND                 \\  
 DF Tau   & 20 Dec 2015 & -                 & -                 & -                 & ND                & ND               & ND                 \\     
          & 08 Dec 2018 & -7.81 $\pm$ 2.51  & 37.59 $\pm$ 4.70  & 9.80  $\pm$ 0.90  & ND                & ND               & ND                 \\
 DG Tau   & 19 Dec 2015 & -                 & -                 & -                 & -17.09 $\pm$ 2.19 & 14.99 $\pm$ 2.12 & 235.00 $\pm$ 22.60 \\
          & 29 Oct 2017 & -6.80 $\pm$ 0.40  & 16.27 $\pm$ 0.19  & 205.00 $\pm$ 4.60 & -7.80  $\pm$ 0.96 & 14.20 $\pm$ 1.26 & 198.50 $\pm$ 12.70 \\
 DH Tau   & 02 Nov 2019 & 1.86 $\pm$ 0.42   & 44.54 $\pm$ 1.16  & 6.60 $\pm$ 0.10   & ND                & ND               & ND                 \\
 IQ Tau   & 02 Nov 2019 & 1.84  $\pm$ 4.89  & 25.42 $\pm$ 13.39 & 21.50 $\pm$ 5.60  &  3.35  $\pm$ 2.52 & 15.05 $\pm$ 3.04 & 27.60 $\pm$ 0.70   \\  
 UX Tau   & 26 Gen 2020 & -2.00 $\pm$ 0.51  & 27.67 $\pm$ 2.18  & 48.50 $\pm$ 2.40  & -6.03 $\pm$ 1.13  & 11.24 $\pm$ 2.66 & 22.60 $\pm$ 4.10   \\  
 DK Tau   & 08 Dec 2018 & -2.39 $\pm$ 9.84  & 61.84 $\pm$ 18.55 & 18.00 $\pm$ 3.00  & ND                & ND               & ND                 \\     
 GG Tau   & 09 Dec 2018 & -0.40 $\pm$ 2.57  & 20.56 $\pm$ 5.83  & 10.50 $\pm$ 2.30  &  1.72  $\pm$ 3.97 & 22.52 $\pm$ 6.96 & 32.70 $\pm$ 4.80   \\
 UZ Tau   & 09 Dec 2018 & -0.10 $\pm$ 5.37  & 54.10 $\pm$ 9.42  & 50.20 $\pm$ 7.50  &  1.27  $\pm$ 2.82 & 41.32 $\pm$ 5.79 & 15.80 $\pm$ 1.90   \\
 GH Tau   & 25 Gen 2020 & -5.00 $\pm$ 4.30  & 68.24 $\pm$ 12.05 & 5.90 $\pm$ 0.70   & ND                & ND               & ND                 \\  
 GI Tau   & 26 Gen 2020 & -1.50 $\pm$ 3.73  & 28.14 $\pm$ 8.40  & 2.80 $\pm$ 0.50   & 1.79 $\pm$ 1.39   & 29.90 $\pm$ 3.27 & 50.60 $\pm$ 4.90   \\  
 DL Tau   & 20 Dec 2015 &  -                & -                 & -                 &  2.62  $\pm$ 2.77 & 15.88 $\pm$ 4.70 & 103.50 $\pm$ 15.60 \\
          & 29 Oct 2017 &  2.70 $\pm$ 3.40  & 22.94 $\pm$ 5.92  & 5.00 $\pm$ 1.20   & -0.60  $\pm$ 1.40 & 19.10 $\pm$ 2.59 & 74.50 $\pm$ 8.60   \\
 HN Tau   & 19 Dec 2015 &  -                & -                 & -                 & -1.48  $\pm$ 2.19 & 42.17 $\pm$ 2.11 & 23.30 $\pm$ 1.00   \\
          & 29 Oct 2017 & -7.50 $\pm$ 1.83  & 47.56 $\pm$ 1.35  & 31.50 $\pm$ 0.60  & -5.33  $\pm$ 3.40 & 37.59 $\pm$ 1.85 & 18.60 $\pm$ 1.00   \\
 CI Tau   & 09 Dec 2018 & -1.48 $\pm$ 2.00  & 18.66 $\pm$ 2.03  & 2.70 $\pm$ 4.00   & ND                & ND               & ND                 \\
 HL Tau   & 24 Nov 2016 &  -                & -                 & -                 & -8.72  $\pm$ 3.00 & 11.97 $\pm$ 0.25 & -                  \\
 XZ Tau   & 14 Mar 2017 & -0.89 $\pm$ 1.91  & 13.08 $\pm$ 3.78  & -                 & -5.79  $\pm$ 1.78 & 16.87 $\pm$ 0.53 & -			        \\	
 GK Tau   & 02 Nov 2019 & -5.41 $\pm$ 2.03  & 36.59 $\pm$ 0.92  & 11.80 $\pm$ 0.20  & ND                & ND               & ND                 \\
 DN Tau   & 01 Nov 2019 & -4.34 $\pm$ 2.04  & 45.23 $\pm$ 1.07  & 9.90 $\pm$ 0.20   & ND                & ND               & ND                 \\           
 HQ Tau   & 01 Nov 2019 & -6.45 $\pm$ 2.14  & 48.78 $\pm$ 1.95  & 7.40 $\pm$ 0.20   & ND                & ND               & ND                 \\
 CoKu HP  & 25 Gen 2020 & ND                & ND                & ND                & ND                & ND               & ND                 \\  
 DO Tau   & 19 Dec 2015 &  -                & -                 & -                 & -1.38  $\pm$ 2.43 & 9.20  $\pm$ 1.13 & 49.90 $\pm$ 6.00   \\
          & 13 Nov 2017 & -17.30 $\pm$ 2.75 & 34.60 $\pm$ 4.09  & 23.10 $\pm$ 1.80  & -17.30 $\pm$ 1.53 & 11.50 $\pm$ 2.69 & 60.00 $\pm$ 9.60   \\
          & 26 Gen 2020 & -14.30 $\pm$ 3.17 & 24.83 $\pm$ 7.69  & 24.50 $\pm$ 3.30  & -15.70 $\pm$ 2.10 & 11.10 $\pm$ 1.51 & 58.80 $\pm$ 6.00   \\  
 DQ Tau   & 02 Nov 2019 & -4.89 $\pm$ 2.08  & 26.95 $\pm$ 1.81  & 30.00 $\pm$ 0.90  & ND                & ND               & ND                 \\ 
 DR Tau   & 25 Gen 2020 & 0.90 $\pm$ 1.48   & 19.85 $\pm$ 1.41  & 15.00 $\pm$ 0.90  & 1.75 $\pm$ 0.99   & 20.62 $\pm$ 2.33 & 61.30 $\pm$ 5.70   \\  
 DS Tau   & 01 Nov 2019 & 3.76 $\pm$ 2.22   & 52.52 $\pm$ 2.74  & 4.60 $\pm$ 0.20   &  1.45  $\pm$ 2.65 & 26.69 $\pm$ 4.10 & 3.70 $\pm$ 0.50    \\
 UY Aur   & 08 Dec 2018 & -0.5 $\pm$ 1.94   & 18.19 $\pm$ 3.43  & 27.10 $\pm$ 3.70  & -0.34  $\pm$ 1.70 & 12.70 $\pm$ 0.52 & 107.10 $\pm$ 6.00  \\
 GM Aur   & 09 Dec 2018 & -0.89 $\pm$ 3.95  & 11.01 $\pm$ 4.87  & 17.80 $\pm$ 2.20  & -1.39  $\pm$ 1.69 & 17.65 $\pm$ 2.82 & 15.80 $\pm$ 2.20   \\
 MWC 480  & 01 Nov 2019 & -13.20 $\pm$ 2.16 & 30.47 $\pm$ 2.06  & 38.80 $\pm$ 2.20  & ND                & ND               & ND                 \\ 
 V836 Tau & 02 Nov 2019 & -4.23 $\pm$ 2.05  & 42.81 $\pm$ 1.16  & 4.80 $\pm$ 0.10   & ND                & ND               & ND                 \\
 RW Aur A & 13 Nov 2017 &  ND               & ND                & ND                & -2.60  $\pm$ 3.01 & 16.61 $\pm$ 5.23 & 72.00 $\pm$ 18.60  \\
 CQ Tau   & 13 Nov 2017 & 3.30 $\pm$ 3.37   & 29.34 $\pm$ 4.55  & 16.70 $\pm$ 2.00  & ND                & ND               & ND                 \\    
\hline
\end{tabular}
\begin{quotation}
\textbf{Notes.} Peak velocity ($v_p$) and FWHM are in $\rm km$ $\rm s^{-1}$, while peak intensity ($\rm I_p$) is in $\rm erg$ $\rm s^{-1}$ $\rm cm^{-2}$ $\AA^{-1}$ $10^{-15}$. ND: profile not-detected, "-": spectrum not-acquired.
\end{quotation}
\end{table*} 


==> Tables/ORDERED_by_coordinates/LineKinematicParameters_all_components.tex <==
\begin{table*}
\center
\caption{\label{tab:KinematicParametersAll} Line kinematic parameters of the Gaussian components having $\rm |v|>30$ $\rm km$ $\rm s^{-1}$ for the \oi\ and \htwo\ profiles.}
\begin{tabular}{lc|ccc|ccc}
\hline
\hline
          &             & \multicolumn{3}{c}{\oi}                     & \multicolumn{3}{c}{\htwo}		                                 \\	
Source    & Obs Date    & $\rm v_p$               & $\rm FWHM$             & $\rm I_p$            & $\rm v_p$              & $\rm FWHM$             & $\rm I_p$           \\
\hline   
 CW Tau   & 12-08-2018  & -12.19  $\pm$ 17.34 & 105.94 $\pm$ 39.52 & 8.90  $\pm$ 2.60  & ND                 & ND                 & ND                \\  
          &             & -117.00 $\pm$ 13.23 & 62.35  $\pm$ 45.80 & 7.10  $\pm$ 2.80  & ND                 & ND                 & ND                \\  
 V409 Tau & 01-26-2020  & -50.05 $\pm$ 3.84   & 68.24 $\pm$ 10.93  & 2.30  $\pm$ 0.30  & ND                 & ND                 & ND                \\
          &             & -123.10 $\pm$ 6.49  & 44.67 $\pm$ 20.96  & 0.80  $\pm$ 0.20  & ND                 & ND                 & ND                \\ 
 DD Tau   & 12-19-2015  & -                   & -                  & -                 & ND                 & ND                 & ND                \\
 BP Tau   & 01-26-2020  & 35.4 $\pm$ 6.51     & 28.15 $\pm$ 12.88  & 5.90  $\pm$ 2.10  & ND                 & ND                 & ND                \\  
          &             & -29.5 $\pm$ 5.76    & 30.50 $\pm$ 19.55  & 5.60  $\pm$ 2.00  & ND                 & ND                 & ND                \\  
 RY Tau   & 11-13-2017  & -56.90 $\pm$ 14.14  & 56.94 $\pm$ 15.75  & 25.20 $\pm$ 7.10  & ND                 & ND                 & ND                \\
 FT Tau   & 01-25-2020  & -105.00 $\pm$ 13.00 & 94.16 $\pm$ 20.74  & 1.00  $\pm$ 0.20  & ND                 & ND                 & ND                \\     
 IP Tau   & 12-09-2018  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\
 DF Tau   & 12-08-2018  & 128.09  $\pm$ 5.25  & 54.10 $\pm$ 13.53  & 4.80  $\pm$ 1.00  & ND                 & ND                 & ND                \\
          &             & 32.94   $\pm$ 13.20 & 70.59 $\pm$ 20.32  & 3.90  $\pm$ 1.00  & ND                 & ND                 & ND                \\
          &             & -54.82  $\pm$ 3.05  & 64.70 $\pm$ 5.47   & 10.60 $\pm$ 1.00  & ND                 & ND                 & ND                \\
          &             & -107.10 $\pm$ 1.55  & 42.31 $\pm$ 6.68   & 12.50 $\pm$ 1.20  & ND                 & ND                 & ND                \\
 DG Tau   & 12-19-2015  & -                   & -                  & -                 & -32.48 $\pm$ 5.33  & 11.89 $\pm$ 9.17   & 45.00 $\pm$ 26.0  \\
          & 10-29-2017  & -22.50 $\pm$ 0.63   & 21.03 $\pm$ 0.92   & 104.00 $\pm$ 3.50 & -23.18 $\pm$ 8.47  & 15.50 $\pm$ 13.22  & 17.50 $\pm$ 13.70 \\
          &             & -61.00 $\pm$ 0.79   & 77.67 $\pm$ 0.93   & 135.50 $\pm$ 2.20 & ND                 & ND                 & ND                \\
          &             & -129.30 $\pm$ 1.09  & 51.98 $\pm$ 0.60   & 254.00 $\pm$ 1.70 & ND                 & ND                 & ND                \\
 DH Tau   & 11-02-2019  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\
 IQ Tau   & 11-02-2019  & -29.97 $\pm$ 1.18   & 34.04 $\pm$ 3.02   & 69.50 $\pm$ 1.20  & -11.45 $\pm$ 2.67  & 11.22 $\pm$ 2.49   & 24.50 $\pm$ 1.00  \\  
 UX Tau   & 01-26-2020  & 23.50 $\pm$ 5.74    & 61.17 $\pm$ 20.35  & 8.80  $\pm$ 1.90  & ND                 & ND                 & ND                \\ 
 DK Tau   & 12-08-2018  & -                   & -                  & -                 & ND                 & ND                 & ND                \\    
 GG Tau   & 12-09-2018  & -20.00 $\pm$ 8.61   & 13.89 $\pm$ 22.41  & 2.40  $\pm$ 2.30  & -14.82 $\pm$ 7.60  & 5.28 $\pm$ 7.08    & 12.50 $\pm$ 8.80  \\
 UZ Tau   & 12-09-2018  & -72.00 $\pm$ 1.54   & 63.53 $\pm$ 8.14   & 46.00 $\pm$ 6.00  & ND                 & ND                 & ND                \\
 GH Tau   & 01-25-2020  & -69.00 $\pm$ 12.65  & 47.03 $\pm$ 32.71  & 1.50  $\pm$ 0.60  & ND                 & ND                 & ND                \\
 GI Tau   & 01-26-2020  & 42.05 $\pm$ 5.94    & 35.23 $\pm$ 13.59  & 2.00  $\pm$ 0.50  & ND                 & ND                 & ND                \\ 
          &             & -43.00 $\pm$ 7.29   & 62.35 $\pm$ 14.35  & 2.00  $\pm$ 0.40  & ND                 & ND                 & ND                \\   
 DL Tau   & 12-20-2015  & -                   & -                  & -                 & -12.70 $\pm$ 7.58  & 7.13 $\pm$ 7.51    & 21.50 $\pm$ 20.10 \\
          & 10-29-2017  & 20.00 $\pm$ 21.73   & 38.53 $\pm$ 36.62  & 1.50  $\pm$ 0.90  & -17.95 $\pm$ 5.24  & 10.28 $\pm$ 7.56   & 18.00 $\pm$ 11.60 \\
          &             & -18.80 $\pm$ 6.90   & 13.42 $\pm$ 21.03  & 3.10  $\pm$ 1.30  & ND                 & ND                 & ND                \\
          &             & -68.00 $\pm$ 13.70  & 94.15 $\pm$ 31.60  & 2.70  $\pm$ 0.60  & ND                 & ND                 & ND                \\
          &             & -164.50 $\pm$ 11.89 & 85.91 $\pm$ 19.19  & 3.40  $\pm$ 8.70  & ND                 & ND                 & ND                \\             
 HN Tau   & 12-19-2015  & -                   & -                  & -                 & ND                 & ND                 & ND                \\
          & 10-29-2017  & -                   & -                  & -                 & ND                 & ND                 & ND                \\
 CI Tau   & 12-09-2018  & -19.40 $\pm$ 1.85   & 11.23 $\pm$ 5.61   & 1.30  $\pm$ 0.30  & ND                 & ND                 & ND                \\
 HL Tau   & 11-24-2016  & -                   & -                  & -                 & ND                 & ND                 & ND                \\
 XZ Tau   & 03-14-2017  & -                   & -                  & -                 & ND                 & ND                 & ND                \\	
 GK Tau   & 11-02-2019  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\
 DN Tau   & 11-01-2019  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\           
 HQ Tau   & 11-01-2019  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\
 CoKu HP  & 01-25-2020  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\ 
 DO Tau   & 12-19-2015  & -                   & -                  & -                 & -13.39 $\pm$ 2.80  & 7.13 $\pm$ 2.52    & 19.50 $\pm$ 7.20  \\
          & 11-13-2017  & -89.00 $\pm$ 1.80   & 56.44 $\pm$ 2.38   & 41.00 $\pm$ 1.40  & -28.30 $\pm$ 4.65  & 5.75 $\pm$ 4.80    & 22.00 $\pm$ 18.00 \\
          &             & -102.30 $\pm$ 0.74  & 23.96 $\pm$ 1.09   & 59.30 $\pm$ 2.10  & ND                 & ND                 & ND                \\
          & 01-26-2020  & -74.00 $\pm$ 3.95   & 69.42 $\pm$ 14.25  & 26.00 $\pm$ 2.90  & ND                 & ND                 & ND                \\
          &             & -106.60 $\pm$ 0.31  & 25.30 $\pm$ 2.58   & 84.20 $\pm$ 2.60  & ND                 & ND                 & ND                \\
 DQ Tau   & 11-02-2019  & -18.90 $\pm$ 1.99   & 63.53 $\pm$ 5.69   & 13.70 $\pm$ 1.00  & ND                 & ND                 & ND                \\ 
          &             & -78.15 $\pm$ 7.43   & 30.97 $\pm$ 16.11  & 4.10  $\pm$ 1.30  & ND                 & ND                 & ND                \\ 
 DR Tau   & 01-25-2020  & -19.5 $\pm$ 9.62    & 70.60 $\pm$ 24.73  & 3.30  $\pm$ 0.60  & ND                 & ND                 & ND                \\   
 DS Tau   & 11-01-2019  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\
 UY Aur   & 12-08-2018  & -20.5 $\pm$ 7.86    & 23.17 $\pm$ 12.27  & 8.40  $\pm$ 4.40  & ND                 & ND                 & ND                \\
          &             & -30.00 $\pm$ 19.79  & 164.82 $\pm$ 64.17 & 9.50  $\pm$ 2.00  & ND                 & ND                 & ND                \\     
 GM Aur   & 12-09-2018  & ND                  & ND                 & ND                & -15.53 $\pm$ 3.84  & 4.19 $\pm$ 2.60    & 4.30 $\pm$ 2.60   \\
 MWC 480  & 11-01-2019  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\ 
 V836 Tau & 11-02-2019  & ND                  & ND                 & ND                & ND                 & ND                 & ND                \\
 RW Aur A & 11-13-2017  & 111.60 $\pm$ 7.93   & 73.95 $\pm$ 15.52  & 75.50 $\pm$ 13.70 & ND                 & ND                 & ND                \\
          &             & -90.90 $\pm$ 8.92   & 211.28 $\pm$ 19.75 & 108.00 $\pm$ 9.80 & -20.85 $\pm$ 8.03  & 15.18 $\pm$ 5.64   & 36.00 $\pm$ 20.20 \\
          &             & -172.10 $\pm$ 9.93  & 73.85 $\pm$ 22.51  & 65.00 $\pm$ 16.30 & -24.00 $\pm$ 13.04 & 179.67 $\pm$ 14.86 & 38.00 $\pm$ 5.40  \\
 CQ Tau   & 11-13-2017  & -23.90 $\pm$ 3.95   & 18.06 $\pm$  6.73  & 81.50 $\pm$ 33.30 & ND                 & ND                 & ND                \\
\hline
\end{tabular}
\begin{quotation}
\textbf{Notes.} Peak velocity ($v_p$) and FWHM are in $\rm km$ $\rm s^{-1}$, while peak intensity ($\rm I_p$) is in $\rm erg$ $\rm s^{-1}$ $\rm cm^{-2}$ $\AA^{-1}$ $10^{-15}$. ND: profile not-detected, "-": spectrum not-acquired.
\end{quotation}
\end{table*} 


==> Tables/ORDERED_by_coordinates/SourceProperties.tex <==
\begin{table*}
\small
\center
\caption{\label{tab:SourceProperties} Source properties.}
\begin{tabular}{lcccccccc}
\hline
Source    & RA         & Dec           & d           & SpT          & $A_v$          & $L_\star$      & $M_{\star}$   & $i_{disk}$      \\
          & [J2000]    & [J2000]       & [pc]        &              & [mag]          & [$L_{\odot}$]  & [$M_{\odot}$] & [deg]           \\
\hline
\hline   
 BP Tau   & 04:19:15.83 & +29:06:26.93 & 129          & M0.5$^{(1)}$ & 0.45$^{(1)}$   & 0.42$^{(1)}$   & 0.52$^{(2)}$  & 38.2$^{(2)}$    \\
 CI Tau   & 04:33:52.01 & +22:50:30.09 & 158 		  & K5.5$^{(1)}$ & 1.90$^{(1)}$   & 0.63$^{(1)}$   & 0.90$^{(3)}$  & 50.0$^{(4)}$    \\
 CoKu HP  & 04:35:54.15 & +22:54:13.40 & 166          & G2$^{(1)}$   & 2.55$^{(1)}$   & 6.92$^{(1)}$   & ...           & 50$^{(5)}$      \\ 
 CQ Tau   & 05:35:58.47 & +24:44:54.09 & 163 		  & F5$^{(6)}$   & 1.89$^{(7)}$   & 11.94$^{(7)}$  & 1.75$^{(7)}$  & 29$^{(8)}$      \\
 CW Tau   & 04:14:17.00 & +28:10:57.76 & 132 		  & K3.0$^{(1)}$ & 1.80$^{(1)}$   & 0.45$^{(1)}$   & 1.01$^{(3)}$  & 59$^{(9)}$      \\
 DD Tau   & 04:18:31.13 & +28:16:29.16 & 123 		  & M4.8$^{(1)}$ & 0.75$^{(1)}$   & 0.29$^{(1)}$   & 0.13$^{(1)}$  & ...             \\
 DF Tau   & 04:27:02.79 & +25:42:22.46 & 124 		  & M2.7$^{(1)}$ & 0.10$^{(1)}$   & 0.91$^{(1)}$   & 0.32$^{(3)}$  & 52$^{(3)}$      \\ 
 DG Tau   & 04:27:04.69 & +26:06:16.04 & 121 		  & K7.0$^{(1)}$ & 1.60$^{(1)}$   & 0.51$^{(1)}$   & 0.76$^{(3)}$  & 37$^{(9)}$      \\
 DH Tau   & 04:29:41.56 & +26:32:58.27 & 135 		  & M2.3$^{(1)}$ & 0.65$^{(1)}$   & 0.22$^{(1)}$   & 0.41$^{(3)}$  & 16.9$^{(2)}$    \\
 DK Tau   & 04:30:44.25 & +26:01:24.47 & 128 		  & K8.5$^{(1)}$ & 0.70$^{(1)}$   & 0.54$^{(1)}$   & 0.68$^{(3)}$  & 12.8$^{(2)}$    \\
 DL Tau   & 04:33:39.08 & +25:20:38.10 & 159 		  & K5.5$^{(1)}$ & 1.80$^{(1)}$   & 0.50$^{(1)}$   & 0.98$^{(2)}$  & 45.0 $^{(2)}$   \\
 DN Tau   & 04:35:27.38 & +24:14:58.91 & 128 		  & M0.3$^{(1)}$ & 0.55$^{(1)}$   & 0.83$^{(1)}$   & 0.55$^{(3)}$  & 35.2$^{(4)}$    \\
 DO Tau   & 04:38:28.59 & +26:10:49.47 & 139 		  & M0.3$^{(1)}$ & 0.75$^{(1)}$   & 0.22$^{(1)}$   & 0.59$^{(2)}$  & 27.6 $^{(2)}$   \\
 DQ Tau   &	04:46:53.06 & +17:00:00.13 & 197 		  & M0.6$^{(1)}$ & 1.40$^{(1)}$   & 1.17$^{(2)}$   & 1.61$^{(2)}$  & 16.1 $^{(2)}$   \\
 DR Tau   & 04:47:06.21 & +16:58:42.81 & 196          & K6c$^{(1)}$  & 0.45$^{(1)}$   & 0.32$^{(1)}$   & 0.93$^{(2)}$  & 5.4$^{(2)}$     \\
 DS Tau	  & 04:47:48.59 & +29:25:11.19 & 159 		  & M0.4$^{(1)}$ & 0.25$^{(1)}$   & 0.19$^{(1)}$   & 0.69$^{(3)}$  & 65.2$^{(4)}$    \\
 FT Tau   & 04:23:39.19 & +24:56:14.11 & 128          & M2.8$^{(1)}$ & 1.30$^{(1)}$   & 0.18$^{(1)}$   & 0.34$^{(2)}$  & 35.5$^{(2)}$    \\
 GG Tau   & 04:32:30.33 & +17:31:40.83 & 140 		  & K7.5$^{(1)}$ & 1.00$^{(1)}$   & 1.41$^{(1)}$   & 0.62$^{(1)}$  & 35$^{(10)}$     \\
 GH Tau   & 04:33:06.22 & +24:09:33.63 & 130$^{(11)}$ & M2.3$^{(1)}$ & 0.40$^{(1)}$   & 0.64$^{(1)}$   & 0.36$^{(12)}$  & ...            \\
 GI Tau   & 04:33:34.06 & +24:21:17.07 & 130          & M0.4$^{(1)}$ & 2.05$^{(1)}$   & 0.56$^{(1)}$   & 0.52$^{(2)}$  & 43.8$^{(2)}$    \\
 GK Tau   &	04:33:34.56 & +24:21:05.85 & 129 		  & K6.5$^{(1)}$ & 1.50$^{(1)}$   & 0.93$^{(1)}$   & 0.69$^{(3)}$  & 40.2$^{(2)}$    \\
 GM Aur   & 04:55:10.98 & +30:21:59.37 & 159 		  & K6 $^{(3)}$  & 0.30$^{(1)}$   & 0.49$^{(1)}$   & 0.88$^{(3)}$  & 53.21 $^{(13)}$ \\
 HL Tau   & 04:31:38.44 & +18:13:57.65 & 140 		  & K3c$^{(1)}$  & 2.50$^{(1)}$   & 0.14$^{(1)}$   & 1.8$^{(14)}$  & 47$^{(14)}$     \\
 HN Tau   & 04:33:39.36 & +17:51:52.30 & 145 		  & K3$^{(1)}$   & 1.15$^{(1)}$   & 0.17$^{(1)}$   & 1.53$^{(2)}$  & 69.8 $^{(2)}$   \\
 HQ Tau   & 04:35:47.33 & +22:50:21.64 & 158 		  & K2.0$^{(1)}$ & 2.60$^{(1)}$   & 4.47$^{(1)}$   & 1.53$^{(3)}$  & 53.8$^{(2)}$    \\
 IP Tau   & 04:24:57.08 & +27:11:56.54 & 130 		  & M0.6$^{(1)}$ & 0.75$^{(1)}$   & 0.39$^{(1)}$   & 0.59$^{(3)}$  & 45.2$^{(4)}$    \\
 IQ Tau   & 04:29:51.56 & +26:06:44.85 & 131 		  & M1.1$^{(1)}$ & 0.85$^{(1)}$   & 0.24$^{(1)}$   & 0.50 $^{(2)}$ & 62.1$^{(2)}$    \\
 MWC480   &	04:58:46.26 & +29:50:36.99 & 161 		  & A4.5$^{(4)}$ & 0.10 $^{(2)}$  & 17.38$^{(1)}$  & 1.91 $^{(2)}$ & 36.5 $^{(2)}$   \\
 RW Aur A &	05:07:49.54 & +30:24:05.07 & 163 		  & K0$^{(1)}$   & 0-2$^{(1,15)}$ & 0.72$^{(1)}$   & 1.20$^{(2)}$  & 55.1 $^{(2)}$   \\	
 RY Tau   & 04:21:57.41 & +28:26:35.53 & 128 		  & F7$^{(4)}$   & 1.85$^{(1)}$   & 10.71$^{(1)}$  & 2.04$^{(2)}$  & 65.0 $^{(2)}$   \\
 UX Tau   & 04:30:04.00 & +18:13:49.43 & 139$^{(11)}$ & M1.9$^{(1)}$ & 0.40$^{(1)}$   & 0.37$^{(1)}$   & 1.51$^{(3)}$  & 39.0$^{(12)}$   \\
 UY Aur   & 04:51:47.39 & +30:47:13.55 & 155 		  & K7.0$^{(1)}$ & 1.00$^{(1)}$   & 0.85$^{(1)}$   & 0.65 $^{(2)}$ & 23.5 $^{(2)}$   \\
 UZ Tau   & 04:32:43.02 & +25:52:30.90 & 131 		  & M1.9$^{(1)}$ & 0.90$^{(1)}$   & 0.40$^{(1)}$   & 1.23$^{(2)}$  & 56.1 $^{(2)}$   \\
 V409 Tau & 04:18:10.78 & +25:19:57.38 & 131          & M0.6$^{(1)}$ & 1.00$^{(1)}$   & 0.66$^{(1)}$   & 0.50$^{(2)}$  & 69.3$^{(2)}$    \\
 V836 Tau & 05:03:06.60 & +25:23:19.60 & 169 		  & M0.8$^{(1)}$ & 0.60$^{(1)}$   & 0.30$^{(1)}$   & 0.58$^{(3)}$  & 43.1 $^{(2)}$   \\
 XZ Tau   & 04:31:40.09 & +18:13:56.64 & 144$^{(11)}$ & M2$^{(16)}$  & 1.40$^{(16)}$   & 0.42$^{(16)}$   & 0.36$^{(16)}$  & 35$^{(17)}$  \\
 \hline
\end{tabular}
\begin{quotation}
\textbf{Notes.} The distance for each target is computed from the \emph{Gaia} DR2 parallax \citep{Gaia2018}.

\textbf{References.} $^{(1)}$\citet{Herczeg2014}, $^{(2)}$\citet{Long2019}, $^{(3)}$\citet{Simon2016}, $^{(4)}$\citet{Long2018}, $^{(5)}$\citet{Bouvier1995}, $^{(6)}$\citet{Varga2018}, $^{(7)}$\citet{Villebrun2019}, $^{(8)}$\citet{Chapillon2008}, $^{(9)}$\citet{Bacciotti2018}, $^{(10)}$\citet{Phuong2018}, $^{(11)}$\citet{Akeson2019}, $^{(12)}$\citet{Banzatti2019}, $^{(13)}$\citet{Huang2020}, $^{(14)}$\citet{Yen2019}, $^{(15)}$\citet{Koutoulaki2019}, $^{(16)}$\citet{Hartigan2003}, $^{(17)}$\citet{Osorio2016}.
\end{quotation}
\end{table*} 


==> Tables/ORDERED_by_coordinates/h2_properties.tex <==
\begin{table*}
\center
\caption{\label{tab:H2properties} \htwo\ emission properties.}
\begin{tabular}{lcclll}
\hline
\\
Source    & \htwo\ profile$^a$        & [OI] profile$^a$     & $i_{disk}$[deg]  &  Spatial information & Ref.\\
\\
\hline
\hline
\\
\multicolumn{6}{c}{Sources with $v_p$(\htwo) $>|3|$\,\kms} \\
\\
\hline   
 DD Tau  & D & ...    &        & [OI] HV jet  & (1)\\
 DG Tau  & D & D/HVC  & 37     & \htwo\ extended, wind   & (2),(3) \\  
 HN Tau  & S & D/HVC  & 69.8   &  &  \\
 HL Tau  & S & ...    & 47.    &  [OI] HV jet,  \htwo\ extended, wind  &  (4),(5)\\
 XZ Tau  & S & D/HVC  &  35    &  \htwo\ extended, wind   & (2)\\  
 DO Tau  & D & S/HVC  & 27.6   &  &  \\
 UX Tau  & S & S/HVC  &  39    &  [OI] Very broad component, TD(ALMA) &  \\ %BVC corrected +36 km/s
\hline
\\
\multicolumn{6}{c}{Sources with $v_p$(\htwo) $<|3|$\,\kms}\\
\\
\hline
GG Tau  & D & S/HVC  & 35    & \htwo\ extended, disk/infall streams & (6) \\ %BVC corrected +36 km/s
UZ Tau  & S & S/HVC  & 56.1  & TD(ALMA)   & (7) \\
IQ Tau  & D & S/HVC  & 62.1  &            &  \\
DL Tau  & D & D/HVC  & 45    &     &  \\
DS Tau  & S & S      & 65.2  &  &  \\
UY Aur  & S & D/HVC  & 23.5  &  \htwo\ extended, wind, binary & (6) \\
GM Aur  & S & S      & 53.21 &  \htwo\ compact, disk; TD(ALMA) & (6)  \\
BP Tau  & S & D/HVC? & 38.9  & pTD &\\
GI Tau  & S & D/HVC  & 43.8  & &\\
DR Tau  & S & S/HVC  & 5     & &\\ %BVC corrected 224 km/s
\hline
\multicolumn{6}{c}{Summary of \htwo detections) }\\
 \hline \\
\multicolumn{3}{l}{\htwo\, in winds candidates}  & \multicolumn{3}{l}{15 sources}\\
\multicolumn{3}{l}{\htwo\, in disks candidates}  & \multicolumn{3}{l}{2 sources}\\
\hline
\hline \\
\multicolumn{6}{c}{Sources with no \htwo\ detections} \\
\\
 \hline
CW Tau     & ... & D/HVC     & 59   & G-type  &  \\
RY Tau     & ... & S/HVC     & 65   & F-type, TD(ALMA) &  (7) \\
IP Tau     & ... & S         & 45.2 & weak OI  at R<1, TD(ALMA)& (7) \\
DF Tau     & ... & D/HVC     & 52   & OI at R<1 &  \\ 
DK Tau     & ... & S         & 12.8 & OI at R<1 &  \\
DH Tau     & ... & S         & 16.9 & OI at R<1 &  \\     
CI Tau     & ... & D         & 50   & OI weak &  \\
GK Tau     & ... & S         & 40.2 & OI at R <1 &  \\ 
DN Tau     & ... & S         & 35.2 &  OI at R < 1&  \\ 
DQ Tau     & ... & D/HVC     & 16.1 & OI at R <1 &  \\ 
MWC480     & ... & S         & 36.5 & A-type &  \\ 
V836 Tau   & ... & S         & 43.1 & OI at R <1  &  \\
RW Aur A   & ... & D/HVC     & 55.1 & no OI NLVC &  \\
CQ Tau     & ... & D         & 29   & F-type star &  \\
HQ Tau     & ... &  S & 62.1 & OI low S/N? &  \\
V409 Tau ? & ... &  D/HVC    & 69.3 & OI at R <1 &\\
CoKu       & ... &  ...      & 50 & no OI &\\
GH Tau     & ... &  S/HVC    &    & OI at R <1 ? (no inc. angle)&\\
\hline 
\multicolumn{6}{c}{Summary of \htwo non-detections) } \\
 \hline 
\multicolumn{3}{l}{Early type stars}  & \multicolumn{3}{l}{4 sources}\\
\multicolumn{3}{l}{[OI] at R$<$ 1 au}  & \multicolumn{3}{l}{10 sources}\\
\multicolumn{3}{l}{[OI] weak or non-detected}  & \multicolumn{3}{l}{4 sources}\\
\hline \\
\hline
\end{tabular}
\begin{quotation}
\textbf{Notes.} S: LVC with single component profile, D: LVC with double component profile, HVC: presence of at least one high velocity component. The HVC is defined as a component at V$_p >$ 30 km/s, taking also into account corrections for inclination angles. \simo{bisogna scrivere qualcosa sui TD (Reference?). Toglierei la distinzione "pTD".}
\textbf{References.} (1) Hartigan et al. (2004), (2) \citet{Beck2008} , (3) \citet{Agra-Amboage2014}, (4) \citet{Mundt1990}, (5) \citet{Takami2007}, (6) \citet{Beck2019}, (7) \citet{Long2018} \end{quotation}
\end{table*} 

==> Tables/h2_properties.tex <==
\begin{table*}
\center
\caption{\label{tab:H2properties} \htwo\ emission properties.}
\begin{tabular}{lcclll}
\hline
\\
Source    & \htwo\ profile$^a$        & [OI] profile$^a$     & $i_{disk}$[deg]  &  Other information & Ref.\\
\\
\hline
\hline
\\
\multicolumn{6}{c}{Sources with $v_p$(\htwo) $>|3|$\,\kms} \\
\\
\hline   
 DD Tau  & D & ...       &        & \oi\ HV jet                           & (1)      \\
 DG Tau  & D & D/HVC     & 37     & \htwo\ extended, wind                 & (2),(3)  \\  
 DO Tau  & D & S/HVC     & 27.6   &                                       &          \\
 HN Tau  & S & D/HVC     & 69.8   &                                       &          \\
 HL Tau  & S & ...       & 47.    & \oi\ HV jet,  \htwo\ extended, wind   &  (4),(5) \\
 UX Tau  & S & S/HVC     & 39     &  TD ($R_{gap}$=25 au )                 &          \\ %BVC corrected +36 km/s
 XZ Tau  & S & D/HVC     & 35     & \htwo\ extended, wind                 & (2)      \\  
\hline
\\
\multicolumn{6}{c}{Sources with $v_p$(\htwo) $<|3|$\,\kms}\\
\\
\hline
 BP Tau  & S & D/HVC? & 38.9  &                                      &     \\
 DL Tau  & D & D/HVC  & 45    &                                      &     \\
 DR Tau  & S & S/HVC  & 5     &                                      &     \\ %BVC corrected 224 km/s
 DS Tau  & S & S      & 65.2  &                                      &     \\
 GG Tau  & D & S/HVC  & 35    & \htwo\ extended, disk/infall streams & (6) \\ %BVC corrected +36 km/s
 GI Tau  & S & D/HVC  & 43.8  &                                      &     \\
 GM Aur  & S & S      & 53.21 & \htwo\ compact, disk; TD ($R_{gap} \sim$ 30-40 au ) & (6), (7) \\
 IQ Tau  & D & S/HVC  & 62.1  &                                      &     \\
 UY Aur  & S & D/HVC  & 23.5  & \htwo\ extended, wind, binary        & (6) \\
 UZ Tau  & S & S/HVC  & 56.1  & TD ($R_{gap} \sim$ 4.7 au )           & (8)    \\
\hline
\multicolumn{6}{c}{Summary of \htwo\ detections }\\
 \hline \\
\multicolumn{3}{l}{\htwo\, in winds candidates}  & \multicolumn{3}{l}{15 sources}\\
\multicolumn{3}{l}{\htwo\, in disks candidates}  & \multicolumn{3}{l}{2 sources}\\
\hline
\hline \\
\multicolumn{6}{c}{Sources with no \htwo\ detections} \\
\\
 \hline
CI Tau     & ... & D     & 50   & \oi\ weak                      & \\
CoKu       & ... & ...   & 50   & no \oi\                        & \\
CQ Tau     & ... & D     & 29   & F-type star                    & \\
CW Tau     & ... & D/HVC & 59   & G-type                         & \\
DF Tau     & ... & D/HVC & 52   & \oi\ at R<1                    & \\ 
DH Tau     & ... & S     & 16.9 & \oi\ at R<1                    & \\     
DK Tau     & ... & S     & 12.8 & \oi\ at R<1                    & \\
DN Tau     & ... & S     & 35.2 & \oi\ at R < 1                  & \\ 
DQ Tau     & ... & D/HVC & 16.1 & \oi\ at R <1                   & \\ 
GH Tau     & ... & S/HVC &      & \oi\ at R <1 ? (no inc. angle) & \\
GK Tau     & ... & S     & 40.2 & \oi\ at R <1                   & \\ 
HQ Tau     & ... & S     & 62.1 & \oi\ low S/N?                  & \\
IP Tau     & ... & S     & 45.2 & weak OI  at R<1, TD ($R_{gap} \sim$ 21 au )      & (8) \\
MWC480     & ... & S     & 36.5 & A-type                         & \\ 
RW Aur A   & ... & D/HVC & 55.1 & no \oi\ NLVC                   & \\
RY Tau     & ... & S/HVC & 65   & F-type, TD ($R_{gap} \sim$ 6.9 au ) & (8) \\
V409 Tau ? & ... & D/HVC & 69.3 & \oi\ at R <1                   & \\
V836 Tau   & ... & S     & 43.1 & \oi\ at R <1                   & \\
\hline 
\multicolumn{6}{c}{Summary of \htwo\ non-detections } \\
 \hline 
\multicolumn{3}{l}{Early type stars}  & \multicolumn{3}{l}{4 sources}\\
\multicolumn{3}{l}{\oi\ at R$<$ 1 au}  & \multicolumn{3}{l}{10 sources}\\
\multicolumn{3}{l}{\oi\ weak or non-detected}  & \multicolumn{3}{l}{4 sources}\\
\hline \\
\hline
\end{tabular}
\begin{quotation}
\textbf{Notes.} S: LVC with single component profile, D: LVC with double component profile (the other component might have V$_p > |3|$ \kms), HVC: presence of at least one high velocity component. The HVC is defined as a component at V$_p >$ 30 km/s, taking also into account corrections for inclination angles.
\textbf{References.} (1) Hartigan et al. (2004), (2) \citet{Beck2008} , (3) \citet{Agra-Amboage2014}, (4) \citet{Mundt1990}, (5) \citet{Takami2007}, (6) \citet{Beck2019}, (7) \citet{Hornbeck2016}, (8) \citet{Long2018}.  \end{quotation}
\end{table*} 
